Lossy Compression of Scientific Data: Applications Constrains and Requirements

Increasing data volumes from scientific simulations and instruments (supercomputers, accelerators, telescopes) often exceed network, storage, and analysis capabilities. The scientific community's response to this challenge is scientific data reduction. Reduction can take many forms, such as triggering, sampling, filtering, quantization, and dimensionality reduction. This report focuses on a specific technique: lossy compression. Lossy compression retains all data points, leveraging correlations and controlled reduced accuracy. Quality constraints, especially for quantities of interest, are crucial for preserving scientific discoveries. User requirements also include compression ratio and speed. While many papers have been published on lossy compression techniques and reference datasets are shared by the community, there is a lack of detailed specifications of application needs that can guide lossy compression researchers and developers. This report fills this gap by reporting on the requirements and constraints of nine scientific applications covering a large spectrum of domains (climate, combustion, cosmology, fusion, light sources, molecular dynamics, quantum circuit simulation, seismology, and system logs). The report also details key lossy compression technologies (SZ, ZFP, MGARD, LC, SPERR, DCTZ, TEZip, LibPressio), discussing their history, principles, error control, hardware support, features, and impact. By presenting both application needs and compression technologies, the report aims to inspire new research to fill existing gaps.

==> ceresz.tex <==
CereSZ~\cite{ceresz} is a lossy compressor designed based on SZ for the Cerebras CS-2 system. As supercomputers increasingly incorporate new AI chips like Cerebras for scientific computing acceleration, the demand for efficient data compression on these new architectures is growing.

Unlike the CPU and GPU, which are designed based on the control flow architecture and have access to global memory, the computing units on Cerebras construct a dataflow architecture. Each computing unit can only access data from a small local memory and its neighboring units. This restricted memory access presents new challenges in the design and implementation of compression algorithms.

Since the dataflow architecture does not support the maintenance of a global status in the compression process, we adopt a block-wise compression algorithm to distribute the computation. The data is divided into blocks and each block is compressed independently. This approach allows computations on different blocks to be easily mapped onto different computing units on the Cerebras chip, without any need for inter-unit communication. 

We also employ a stage-wise design where the compression process is divided into multiple stages. Each stage only processes the output of the preceding stage. This enables the computation on each block to be mapped to a group of contiguous computing units and parallelized in a pipeline. With the block-wise and stage-wise algorithm design, we can scale out the compression procedure to a 2D mesh of computing units on the Cerebras system. To fully utilize the computing power of Cerebras, CereSZ incorporates two performance optimization techniques. First, to balance the workload among pipeline stages, we divide each stage into finer-grained sub-stages and redistributed evenly into stage groups. Second, we forward data along the computing units to enable parallel execution of multiple pipelines.

The experiments show that CereSZ can achieve an average of 457.35 GB/s and 581.31 GB/s for compression and decompression throughput, respectively. This is 4.97x and 4.84x faster compared to exiting GPU compressors without any losses of data quality.

==> climate-v1.tex <==
%For every application, we consider 1 to 1.5 pages of description:
%Application experts, please write 2/3 describing your Applications, including why compression is needed and the broader importance of your application (what communities will benefit from the development of a dedicated lossy compressor for your application).

%We will ask note-takers to write 1/3 of the content on the collection of needs,  constraints, and Requirements.

%Once done, we will ask the application people to review the needs and constraints and go over the 1 to 1.5 pages for consistency.

 

\subsection{Climate}

\subsubsection{Description}

Understanding the Earth's climate system has long been of interest, particularly as a requirement for better predicting future climate states.  Climate simulation models have become increasingly complex over the decades as computing resources have grown in power and sophistication (e.g., see \cite{washington2005introduction, gettlemanbook}). 
At present, modern Earth system models (ESMs) are widely used to study past, present, and future climate states, and better understanding our changing climate has become an urgent priority for society.  
ESM simulations are well-known for producing enormous amounts of output data, as increases in computational power have enabled finer spatial and temporal resolutions, longer simulations, and larger ensembles.  
And while these advances are desirable for more accurate and realistic simulations, the associated data storage requirements are often prohibitively large, as supercomputing storage capacities have not increased as rapidly as computational power and financial constraints limit the storage capacity available at many institutions \cite{kunkel2014}.

The increasing data generation trend in model-based climate research is simply unsustainable. 
The Coupled Model Intercomparison Projects (CMIPs), which facilitate international ESM comparisons via specific data and experiment specifications, have grown substantially over the years in terms of data volume requirements. The most recent CMIP6 effort resulted in roughly 28 PB from 45 modeling institutes, hosted by the Earth System Grid Federation (ESGF, \cite{ESGF}), while CMIP5 generated 2 PB of data and CMIP3 generated only 40 TB \cite{cmip6}.  
The National Center for Atmospheric Research's (NCAR) contribution to CMIP6  with the Community Earth System Model
(CESM) \cite{cesm2013}, for example, was 2 PB post-processed time series data, and, notably, the vast majority CMIP runs are not even considered high-resolution.
The recent push toward kilometer-scale models (i.e., ``ultra-high" resolution), exemplified by the DYAMOND (DYnamics of the
Atmospheric general circulation Modeled On Non-hydrostatic
Domains) project \cite{Dyamond}, is severely impacted by storage constraints.
In fact, computational and storage costs were so high for the initial DYAMOND atmosphere-only model experiments 
that simulations were limited to 40 days in length 
and 3D variable output was scant.  As an example, the DYAMOND contribution from  SCREAM (Simple Cloud-Resolving E3SM Model \cite{e3sm-scream2023}), run at 3.25 km resolution, was nearly 4.5 TB of data per simulated day \cite{caldwell2021}.
The reality is that climate scientists are often unable to store all of the simulation output that they would like, and this limitation directly impacts climate science research investigations.

Lossy data compression has been proposed by many over the years as a means of mitigating the big data problem in climate (e.g., see \cite{woodring2011, hubbe2013, bicer13, baker2014, kuhn2016, baker2016}.
While certainly an attractive approach, a number of challenges associated with this effort in practice have hindered the widespread acceptance and use of lossy compression in the Earth system modeling community.
First, for ESMs such as the popular CESM, climate scientists' reluctance to lose any information and concerns about the effects of data compression-induced artifacts are justifiable given the societal concerns over future climate and  possible implications of model predictions.
In addition, because of the computational power and storage required by most climate simulation models, large data sets are typically generated by research institutions such as NCAR and then made publicly available for the wider climate research community (e.g., \cite{kay2015, lens2, chang2020}. 
This workflow style means that those generating (and possibly compressing) the output data often do not know how the data will be analyzed. Therefore, identifying particular data characteristics to preserve (e.g., extreme values, subtle shifts in seasonal cycles, changes in gradients) so as not to affect scientific analysis is nontrivial.  
For this reason also, the climate community is taking a cautious approach to adopting lossy compression.
A further challenge is that evaluating the information loss for climate data is non-trivial.  ESMs typically output hundreds (or even thousands) of variables with very different characteristics as well as spatial and temporal dependencies that requires\ the individual treatment
of variables and not a ``one-size-fits-all” approach \cite{baker2014, baker2016, poppick20}.   Indeed, typical compression metrics (e.g., RMSE, PSNR) are simply not able to capture all the kinds of compression artifacts that might be of importance in a wide
variety of analysis settings (e.g., see \cite{baker2014, baker2016, baker2017, Hammerling2019, poppick20, baker2019}).
Finally, we note that the community aspect of large climate data sets means that the lifetime of the data is quite long (possibly ``forever'') and the number of users accessing the data is very large.  In terms of suitable lossy compressors, this aspect means that the climate modelling community is hesitant to use compressor technologies that may not be available/supported for the long haul (rendering old data unreadable) or to require any additional burden on the users in term of reading the compressed data.  (The time and ease of reading data for analysis is extremely important to climate scientists.) Further, ESMs like CESM need fast and parallel I/O for NetCDF files, which can inhibit the use of some lossy compressor technologies, particularly if used to compress when the data is initially output (as opposed to in a post-processing step).  

%Data SSIM \cite{dssim}?

\subsubsection{Lossy compression needs and requirements}


==> light-sources-v1.tex <==
\subsection{Light sources}
\subsubsection{Description}
Over the next few years LCLS-II will deploy new area detectors for high rate ultrafast X-Ray shots.  The device with the highest data volume is a 16 megapixel area detector running at 35kHz, producing \~1TB/s in one of the hutches, with three other hutches having 4 megapixel detectors running at similar rates. The storage costs for this data volume are prohibitive so real-time data-reduction is needed.  Since the experiments vary significantly the entropy of LCLS data also varies, but typically only allows for a factor of about two reduction with lossless compression (due to typically low signal-to-noise) so lossy compression is required.  

\subsubsection{Lossy compression needs and requirements}
Using existing LCLS-I datasets LCLS has studied the effect of lossy compression in crystallography experiments using a custom RoibinSZ algorithm  [RoibinSZ reference] as well as low-intensity and high-intensity SAXS/WAXS experiments using the SZ3 lossy compression algorithm described in this paper.  For the former LCLS has achieved a factor of 90 reduction while for the latter LCLS has achieved a factor of 9 reduction without compromising the physics results.  LCLS has also begun investigating the LC compression package described in this paper.  Since the reduction must be done in real-time LCLS has started benchmarking the performance of the SAXS/WAXS compression in the LCLS-II data acquisition system.  Measurements indicate that LCLS would need close to 1000 64-core nodes to reduce the data volume with SZ3 which LCLS feels is too large to be maintainable by our small team.  In principle this performance could be increased by batching together the data from several LCLS shots before giving it to the compression, but this coupling of event data would break later software in the chain which needs to distribute different batch sizes to CPU cores doing the analysis.  To alleviate this performance bottleneck LCLS has begun researching running these algorithms on GPUs where LCLS hopes to be able to process \~50GB/s per GPU, requiring only \~20 GPUs for our largest 1TB/s detectors.  LCLS is trying to keep as much of the processing of the data on the GPU as possible, DMAing the data directly from the detector FPGAs to the GPU using GPU-Direct over PCI-express, compressing the data, and then storing the data on our WEKA file system using GPU Direct Storage.  The only high-rate part of the data acquisition path LCLS anticipates needing the CPU for is a software-trigger decision where small data results (e.g. Bragg peaks) are communicated to the trigger-decision machines.


==> tab-summary_bak.tex <==
\begin{sidewaystable*}

\caption{Summary of Application Requirements}\label{tab:requirements}

\centering\renewcommand{\arraystretch}{1.0}

\begin{tabularx}{\textwidth}{|X||lXlXXXXXXX|}
\hline \\
Application        & Needs              & Device                     & Target CR         & Bandwidth Ratio                        & Analysis                         & Longevity                & Mechanism                       & Installation                   & Special needs       & Format \\
\hline \\
Molecular Dynamics & storage            & CPU                        & $>3$              & $>1\times$                             & \textcolor{red}{yes}             & 10 Years                 & C,C++,HDF5                      & Spack, Manual                  & Random Block Access               & Particles \\
\hline \\
Climate            & storage            & CPU $\rightarrow$ GPU      & $2-3\times$l      & $>1\times l$                           & ldcpy                            & indefinite               & python, julia, R, HDF5, pnetcdf & site modules, pip/conda, spack & Uncorrelated Dims                 & Dense $\rightarrow$ Unstructured Grid\\
\hline \\
Light Sources      & throughput+storage & CPU $\rightarrow$ GPU,FPGA & $>10\times$        & Realtime 1TB/s                        & manual $\rightarrow$  automatic  & 10 Years                 & Python, C++                     & conda $\rightarrow$ spack      & Uncorrelated Dims                 & Dense \\
\hline \\
Cosmology          & storage+throughput & GPU                        & $>10\times$        & $>1\times l$                          & \textcolor{red}{yes}             & \textcolor{red}{unknown} & HDF5, C++, python               & Manual                         & Hardware Portable Decompression   & Dense \\
\hline \\
Seismology         & throughput+storage & GPU,CPU                    & $>20\times$        & $>1\times l$                          & \textcolor{red}{yes}             & \textcolor{red}{unknown} & Fortran90, CUDA, Python         & Manual                         & Asynchronous Batching              & Dense \\
\hline \\
Combustion         & storage            & GPU                        & $2\times-5\times$ & not urgent                             & topological descriptors          & 5-10 years               & C++, Python, HDF5               & Manual, pip                    &                                   & Dense \\
\hline \\
Fusion             & storage+throughput & GPU                        & $>5\times$         & not urgent $\rightarrow$ $>1\times l$ & \textcolor{red}{yes}             & Ephmerial                & HDF5 $\rightarrow$ Python       & Manual, site modules, pip      &streaming, provence                & 2D Dense \\
\hline \\
Quantum Circuit    & memory capacity    & GPU,CPU                    & $2\times-10\times$& Realtime 25GB/s                        & conservation laws, distributional& Ephmerial                & Python                          & pip                            &                                   & 20-30D Dense \\
\hline \\
System Logs        & throughput         & CPU                        & $>10\times$        & $>10\times l$                         & \textcolor{red}{yes}             & Ephmerial                & Python                          & pip,conda                      & Queries (\`a la SQL)              & 2D Tables \\
\hline
\end{tabularx}

\end{sidewaystable*}
